Modeling contact binaries, II. The effect of energy transfer

Context. It is common for massive stars to engage in binary interaction. In close binaries, the components can enter a contact phase, where both stars overflow their respective Roche lobes simultaneously. While there exist observational constraints on the stellar properties of such systems, the most detailed stellar evolution models that feature a contact phase are not fully reconcilable with those measurements. Aims. We aim to consistently model contact phases of binary stars in a 1D stellar evolution code. To this end, we develop the methodology to account for energy transfer in the common contact layers. Methods. We implement an approximative model for energy transfer between the components of a contact binary based on the von Zeipel theorem in the stellar evolution code MESA. We compare structure and evolution models with and without this transfer and analyze the implications for the observable properties of the contact phase. Results. Implementing energy transfer helps eliminating baroclinicity in the common envelope between the components of a contact binary, which, if present, would drive strong thermal flows. We find that accounting for energy transfer in massive contact binaries significantly alters the mass ratio evolution and can extend the lifetime of an unequal mass ratio contact system.

==> chapters/CslowET.tex <==
\section{Energy transfer in fast mass transfer phases}
Given the caveat stated in Sect. \ref{ssec:et}, we address whether including ET only when the star is in thermal equilibrium changes the evolution.
To test this, we use the setup for the $19+14M_\odot$ binary as described above, but require for ET to occur the additional condition that:
\begin{equation}\label{eq:slowET}
    \left|\frac{M}{\dot{M}}\right|_{\rm donor} > 10 \tau_{\rm thermal, donor},
\end{equation}
meaning that the mass transfer timescale is at least an order of magnitude larger than the thermal timescale of the donor star.
This will shut of our ET implementation during the fast case A MT phase, while retain it during the slow case A phase.
Figure \ref{fig:slowET} shows the MT rate and mass ratio evolution from the point of RLOF to $L_2$ overflow.
By comparing the ET track with the `slow ET' track, which requires the condition of Eq. \eqref{eq:slowET}, we note that including ET during fast MT phases only slightly changes the evolution of this binary model.
For full ET, the final mass ratio after fast case A is slightly higher, which delays reattachment of the primary, but the slow evolving contact phase is nearly unchanged.
\begin{figure}
    \centering
    \includegraphics{img/slowET.png}
    \caption{Mass transfer rate and mass ratio evolution of the $19+14M_\odot$ binary studied in Sect. \ref{ssec:detailed}. For the purple line labeled `slow ET', we required the additional condition of Eq. \eqref{eq:slowET} for ET to occur.}
    \label{fig:slowET}
\end{figure}
\par
